Printable Aggregate Elements

Aggregating base elements into rigid objects such as furniture or sculptures is a great way for designers to convey a specific look and feel. Unfortunately, there is no existing solution to help model structurally sound aggregates. The challenges stem from the fact that the final shape and its structural properties emerge from the arrangements of the elements, whose sizes are large so that they remain easily identifiable. Therefore there is a very tight coupling between the object shape, structural properties, and the precise layout of the elements. We present the first method to create aggregates of elements that are structurally sound and can be manufactured on 3D printers. Rather than having to assemble an aggregate shape by painstakingly positioning elements one by one, users of our method only have to describe the structural purpose of the desired object. This is done by specifying a set of external forces and attachment points. The algorithm then automatically optimizes a layout of user-provided elements that answers the specified scenario. The elements can have arbitrary shapes: convex, concave, elongated, and can be allowed to deform. Our approach creates connections between elements through small overlaps preserving their appearance, while optimizing for the global rigidity of the resulting aggregate. We formulate a topology optimization problem whose design variables are the positions and orientations of individual elements. Global rigidity is maximized through a dedicated gradient descent scheme. Due to the challenging setting -- number of elements, arbitrary shapes, orientation, and constraints in 3D -- we propose several novel steps to achieve convergence.

==> body/25-formulation.tex <==
\subsection{Formulation}
\label{sec:formulation}

We seek to solve the following constrained optimization problem with respect to the set of parameters $\allDofs$ describing the element arrangement in the output domain:
%
\begin{subequations}
	\label{eq:optimization-problem-def}
	\begin{align}
		\minimize_\allDofs \quad & \objectiveFunction(\allDofs)
		\label{eq:optim:objective-function}\\
		%
		\text{subject to} \quad & \domainFunction(\allDofs) \leq 0
		\label{eq:optim:domain-constraint}\\
		%
		& \allDofs_{\min} \leq \allDofs \leq \allDofs_{\max}
		\label{eq:optim:box-constraints}
	\end{align}
\end{subequations}
%
The object is $\objectiveFunction$, e.g. compliance minimization $\objectiveFunction = \complianceFunc{\allDofs}$.
The constraint $\domainFunction$ forces elements to stay confined to a user-defined output domain, while $\allDofs_{\min}$ and $\allDofs_{\max}$ are box constraints on the element parameters $\allDofs$.
%and $\deformationFunction$ that prevents excessive deformation in elements that can change shape during the optimization.


==> headers/00-fixpdfcompression.tex <==
% fix.jpg compression issue with an acrobat reader
% set pdf version to 1.4

\RequirePackage{pdf14} % https://tex.stackexchange.com/questions/64585/incompatibilities-of-cmap-with-fontenc-hyperref

\pdfminorversion=4
% Try also this alternative:
%\pdfobjcompresslevel=0 % or =1

% \ifxetex
% \special{pdf:minorversion 4}

% \else\ifluatex
% \directlua{
% 	pdf.setminorversion(4)
% }

% \else
% \pdfminorversion=4

% \fi\fi


==> headers/11-linenofix.tex <==
%http://phaseportrait.blogspot.com/2007/08/lineno-and-amsmath-compatibility.html
%Fix for corruption between amsmath and lineno
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
	\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
	\expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
	\renewenvironment{#1}%
	{\linenomath\csname old#1\endcsname}%
	{\csname oldend#1\endcsname\endlinenomath}}%
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
	\patchAmsMathEnvironmentForLineno{#1}%
	\patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
	\patchBothAmsMathEnvironmentsForLineno{equation}%
	\patchBothAmsMathEnvironmentsForLineno{align}%
	\patchBothAmsMathEnvironmentsForLineno{flalign}%
	\patchBothAmsMathEnvironmentsForLineno{alignat}%
	\patchBothAmsMathEnvironmentsForLineno{gather}%
	\patchBothAmsMathEnvironmentsForLineno{multline}%
}


==> headers/12-usebiblatex.tex <==
% Override \bibhang macro defined by acmsiggraph.cls
\let\bibhang\relax

% Use biblatex package
% Keep the bibtex backend because biber is f*cking slow
% Explicit bibtex backend is required; see e.g. http://tex.stackexchange.com/questions/18045/problem-with-compiling-bibtex-no-citation-commands-error
\usepackage[
	%backend=biber,
	backend=bibtex,
	dashed=false,
	giveninits=true, % Show initials for author first names
	isbn=false,
	maxbibnames=9,
	maxcitenames=2,
	parentracker=true,
	sortcites=false,
	sorting=nyt,
	style=authoryear-comp,
	doi=false,
	url=false,
	eprint=false,
	uniquelist=false,
	uniquename=false,
	useprefix=true,
]{biblatex}

% Set bibitem spacing according to acmsiggraph.cls
%\setlength\bibitemsep{1em}
\setlength\bibitemsep{0.5\baselineskip}

\DeclareLanguageMapping{english}{english-apa}

% Replace parentheses by brackets in \parencite citations
% http://tex.stackexchange.com/questions/16765/biblatex-author-year-square-brackets
\makeatletter
\newrobustcmd*{\parentexttrack}[1]{%
	\begingroup
	\blx@blxinit
	\blx@setsfcodes
	\blx@bibopenparen#1\blx@bibcloseparen
	\endgroup}
\AtEveryCite{%
	\let\parentext=\parentexttrack%
	\let\bibopenparen=\bibopenbracket%
	\let\bibcloseparen=\bibclosebracket}
\makeatother

% Remove parenthesis around year in bibliography
% http://tex.stackexchange.com/questions/12254/biblatex-how-to-remove-the-parentheses-around-the-year-in-authoryear-style
\makeatletter
\def\act@on@bibmacro#1#2{%
	\expandafter#1\csname abx@macro@\detokenize{#2}\endcsname
}
\def\patchbibmacro{\act@on@bibmacro\patchcmd}
\def\pretobibmacro{\act@on@bibmacro\pretocmd}
\def\apptobibmacro{\act@on@bibmacro\apptocmd}
\def\showbibmacro{\act@on@bibmacro\show}
\makeatother

\patchbibmacro{date+extrayear}{%
	\printtext[parens]%
	}{%
	\setunit{\addperiod\space}%
	\printtext%
	}{}{
}

% Display last names first in bibliography
\DeclareNameAlias{sortname}{last-first}
\DeclareNameAlias{default}{last-first}

% Use small-caps for author names
\renewcommand{\mkbibnamefamily}[1]{\ifbibliography{\textsc{#1}}{#1}}
\renewcommand{\mkbibnameprefix}[1]{\ifbibliography{\textsc{#1}}{#1}}

% Remove quotes around titles in bibliography
\DeclareFieldFormat[article,inbook,incollection,inproceedings,patent,thesis,unpublished]{title}{#1}

% Remove 'pp.' before pages
\DefineBibliographyStrings{english}{%
	page  = {\ifbibliography{}{p\adddot}},
	pages = {\ifbibliography{}{pp\adddot}},
}

% Remove 'in:' before journals
\renewbibmacro{in:}{}

% Separate author names by a semicolon instead of a simple comma
%\renewcommand*{\multinamedelim}{\addsemicolon\space}
\renewcommand*{\finalnamedelim}{ \ifbibliography{\textsc{and}}{and}\space}

% Make \cite{} behave like \parencite{} with the authoryear style
\renewcommand{\cite}{\autocite}

% Hyphenation penalties for urls
%\setcounter{biburlnumpenalty}{9000} % after numbers (e.g. in DOI)
%\setcounter{biburlucpenalty}{9000} % after all uppercase letters
\setcounter{biburllcpenalty}{9000} % after all lowercase letters

% Replace '-' by \hyphen in .bib file
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{
			\step[fieldsource=title,
				match=\regexp{-},
			replace=\regexp{\\hyphen\{\}}]
			\step[fieldsource=author,
				match=\regexp{-},
			replace=\regexp{\\hyphen\{\}}]
		}
	}
}

